LatentLens: Revealing Highly Interpretable Visual Tokens in LLMs

Transforming a large language model (LLM) into a vision-language model (VLM) can be achieved by mapping the visual tokens from a vision encoder into the embedding space of an LLM. Intriguingly, this mapping can be as simple as a shallow MLP transformation. To understand why LLMs can so readily process visual tokens, we need interpretability methods that reveal what is encoded in the visual token representations at every layer of LLM processing. In this work, we introduce LatentLens, a novel approach for mapping latent representations to descriptions in natural language. LatentLens encodes a large text corpus and stores contextualized token representations for each token in that corpus. Visual token representations are then compared to these contextualized representations and the top-nearest neighbor representations serve as descriptions of the visual token. We evaluate this method on 15 different VLMs, showing that commonly used methods, such as LogitLens, substantially underestimate the interpretability of visual tokens. With LatentLens instead, the majority of visual tokens are interpretable across all studied models and all layers. Qualitatively, we show that the descriptions produced by LatentLens are semantically meaningful and provide more fine-grained interpretations for humans compared to individual tokens. More broadly, our findings contribute new evidence on the alignment between vision and language representations and open up new directions for analyzing the latent representations of LLMs.

==> macros.tex <==
% Commands for commenting and todos
% Only load todonotes if not already loaded (allows main file to set options like [disable])
\makeatletter
\@ifpackageloaded{todonotes}{}{\usepackage{todonotes}}
\makeatother
\usepackage[normalem]{ulem}
\usepackage{xspace}
\usepackage{float} % for [H] figure placement

\setlength{\marginparwidth}{1.5cm}
\makeatletter
\newcommand*\iftodonotes{\if@todonotes@disabled\expandafter\@secondoftwo\else\expandafter\@firstoftwo\fi}  % defines \iftodonotes{<true>}{<false>}, thanks to https://tex.stackexchange.com/questions/126559/conditional-based-on-packageoption
\makeatother
\newcommand{\noindentaftertodo}{\iftodonotes{\noindent}{}}
% Note that these macros accept optional arguments such as size=\small, bordercolor=red, and so on.  Capitalized versions are inline paragraphs instead of margin notes.

% defne the fixme command
\newcommand{\fixme}[2][]{\todo[color=yellow,size=\scriptsize,fancyline,caption={},#1]{#2}} % to mark stuff that you know is missing or wrong when you write the text
\newcommand{\Fixme}[2][]{\fixme[inline,#1]{#2}\noindentaftertodo}

% define the note command
\newcommand{\note}[4][]{\todo[author=#2,color=#3,size=\scriptsize,fancyline,caption={},#1]{#4}} % default note settings, used by macros below.
\newcommand{\response}[1]{\vspace{3pt}\hrule\vspace{3pt}\textbf{#1:}}

% one per co-author
\newcommand{\marius}[2][]{\note[#1]{Marius}{orange!40}{#2}}
\newcommand{\Marius}[2][]{\marius[inline,#1]{#2}\noindentaftertodo}
\newcommand{\mm}[1]{\textcolor{orange}{MM: #1}}
\newcommand{\mariussuggests}[2]{\textcolor{red!20}{\sout{#1}}\textcolor{orange}{mm: #2}}

% one per co-author
\newcommand{\siva}[2][]{\note[#1]{Siva}{blue!40}{#2}}
\newcommand{\Siva}[2][]{\siva[inline,#1]{#2}\noindentaftertodo}
\newcommand{\sr}[1]{\textcolor{blue}{SR: #1}}
\newcommand{\sivasuggests}[2]{\textcolor{blue!20}{\sout{#1}}\textcolor{blue}{sr: #2}}

\newcommand{\benno}[2][]{\note[#1]{Benno}{green!40}{#2}}
\newcommand{\bk}[1]{\textcolor{blue}{BK: #1}}
\newcommand{\de}[2][]{\note[#1]{DE}{blue!40}{#2}}


% one per co-author
\newcommand{\sonia}[2][]{\note[#1]{Sonia}{purple!40}{#2}}
\newcommand{\Sonia}[2][]{\sonia[inline,#1]{#2}\noindentaftertodo}
\newcommand{\sj}[1]{\textcolor{purple}{SJ: #1}}
\newcommand{\soniasuggests}[2]{\textcolor{purple!20}{\sout{#1}}\textcolor{purple}{sj: #2}}

% one per co-author
\newcommand{\oscar}[2][]{\note[#1]{Oscar}{red!40}{#2}}
\newcommand{\Oscar}[2][]{\oscar[inline,#1]{#2}\noindentaftertodo}
% \newcommand{\sj}[1]{\textcolor{red}{OM: #1}}
\newcommand{\oscarsuggests}[2]{\textcolor{red!20}{\sout{#1}}\textcolor{red}{om: #2}}

% other macros

\newcommand{\addcite}{{\color{red}(add citation) }}
\newcommand{\addcites}{{\color{red}(add citations) }}
\newcommand{\writerest}{{\color{red} ... (complete this) }}

\newcommand{\lens}{\textsc{LatentLens}\xspace}
\newcommand{\elens}{EmbeddingLens\xspace}
\newcommand{\logitlens}{LogitLens\xspace}

% Checkmark and crossmark symbols for tables/annotations
\usepackage{pifont}
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%

==> sections/1_intro_realign.tex <==
% -----------------------------------------
\section{Introduction}
\label{sec:introduction}
% -----------------------------------------

Transforming a large language model (LLM) into a vision-language model (VLM) can be as simple as training a linear transformation or shallow MLP that maps visual representations into the embedding space of a frozen LLM \citep[\textit{inter alia}]{tsimpoukelli2021multimodal,merullo2023linearly,liu2023visual,beyer2024paligemma, manas2023mapl}.
% The empirical success of this approach has been repeatedly established, and the downstream performance of VLMs can be further improved by multiple stages of fine-tuning that update different subsets of the model parameters~\citep[]{bai2023qwen,cho2025perceptionlm}.
While VLMs can be further improved via multiple stages of fine-tuning \citep[]{bai2023qwen,cho2025perceptionlm}, the empirical success of frozen LLMs processing non-language inputs raises an important question:
Why is it so easy to adapt an LLM to process data from other modalities?
% Moreover, what is encoded in visual token representations as they are processed by the LLM?
It has been hypothesized that LLMs are ``universal computation engines'' that can process arbitrary modalities with minimal adaptation \citep{lu2022frozen,pmlr-v202-shen23e,garcia-de-herreros-etal-2024-explains}.
Through training on vast amounts of natural language, LLMs may implicitly learn about the physical world, form priors about visual properties \citep{han2025learning}, or even learn a more sophisticated world model \citep{patel2022mapping}.
It has also been argued that separately trained vision and language representations may converge to a shared structure \citep{huh2024position}, which could facilitate training simple projections between them.

% -----------------------------------------
% Figure 1: Place at start of next paragraph for proper wrapfigure flow
\ifworkshop
\begin{wrapfigure}{R}{0.5\textwidth}
   \centering
   \vspace{-0.5em}
   \includegraphics[width=0.48\textwidth]{figures/figure1.pdf}
   \caption{\textbf{Illustration of our method.} \lens compares latent representations of visual tokens to contextualized text representations obtained from full sentence descriptions.}
   \label{fig:teaser}
   \vspace{-1em}
\end{wrapfigure}
\else
\begin{figure}[t]
   \centering
   \includegraphics[width=\figwidth]{figures/figure1.pdf}
   \caption{\textbf{Illustration of our method.} \lens compares latent representations of visual tokens to contextualized text representations obtained from full sentence descriptions.}
   \label{fig:teaser}
\end{figure}
\fi
% https://docs.google.com/drawings/d/1mIhFjTAQVEHZdP9g-K-YEGVShGvKOrgBtfIYt13r3YU/edit?usp=sharing
% -----------------------------------------
However, these hypotheses do not explain how visual representations are integrated inside an LLM and its representation space.
Are the visual tokens processed by an LLM interpretable, i.e., do their representations correspond to semantically meaningful language?
Existing work suggests that visual tokens are rarely interpretable at the input level via nearest neighbors in the language model embedding space~\citep[\elens]{mokady2021clipcap,neo2025towards}.
Recent work has explored the utility of \logitlens, which uses the LLM unembedding matrix~\citep{logitlens}, to interpret and analyze visual token representations \citep{neo2025towards, jiang2025interpreting}.
Finally, training-based methods such as sparse autoencoders \citep{cunningham2023sparse, venhoff2025visual} or supervised probing \citep{fu2025hidden} 
have also been applied to understand what visual representations encode.
However, both embedding-space and training-based methods are inconclusive about the interpretability of visual tokens in LLMs.
%\marius{I simplified this a bit. Let me know what you think.}

In this work, we propose \lens, a novel interpretability method for analyzing latent representations in VLMs.
% a significantly more interpretable and fine-grained interpretability method compared to \logitlens.
\lens is training-free
%, b) inherent --- relying on the LLM's own embeddings and thus provides direct evidence to what extend visual tokens are language-like and c) 
and provides fine-grained sentence-level descriptions of latent representations. 
% (see \Cref{fig:teaser}).
\textbf{Our key insight is that the most natural comparison for visual token representations are \textit{contextual} text representations}, and not the LLM embedding or unembedding matrix.
Thus, \lens compares visual token representations to their nearest neighbors in a large pool of contextualized token representations from intermediate LLM layers.
For example, in~\Cref{fig:teaser}, the visual token of a building yields the nearest neighbor \colorbox{yellow!50}{\textbf{stories}} in the context of ``... building with many \colorbox{yellow!50}{\textbf{stories}}''.

Empirically, we analyze the interpretability of visual token representations across layers for 10 different VLMs.
%, comparing \lens to other training-free approaches such as \elens and \logitlens. 
%as well as one off-the-shelf model (Qwen2-VL-7B-Instruct).
%To automate interpretability annotations, we design an LLM judge.
We find that compared to other training-free approaches (\logitlens and \elens), \lens reveals consistently high interpretability, highlighting that previous methods
% under the right lens, the majority of visual tokens are interpretable --- across all layers and all studied models.
% On the other hand, 
substantially underestimate the interpretability of visual token representations.
Averaged across all models and layers we study, \lens renders 72\% of visual tokens interpretable (according to a VLM-judge).
When using \elens and \logitlens, however, only 30\% and 23\% of visual token representations are labeled as interpretable, respectively.
%(45\% at late layers). DE: weird to only include this detail for LogitLens
Through ablation studies, we provide additional insights about the nature of this interpretable alignment, showing, e.g., that even linear projections lead to interpretable visual token representations.
% We re-train our MLP projector in ablations wrt. the effect of unfreezing the LLM, projection depth or training data.
We also find evidence for a \textit{Mid-Layer Leap} in the learned projection: the visual token representations at the input and early layers align most strongly to contextualized representations from mid-layers (e.g., layers 8--16), suggesting that the learned projection targets semantic rather than lexical representations.
%We term this the }.
We also present qualitative analyses showing that \lens produces rich sentence-level descriptions, unlike \logitlens which might return subwords or next-token predictions.
% Images with rendered text yield particularly clear results where nearest neighbors exactly match the text.

% STEP8: We also make sure this a) holds across ablations and b) off-the-shelf Qwen2-VL-Instruct, c) has interesting effects downstream

% STEP9: Contributions:

% Our primary contributions are:
% \begin{enumerate}
%     \item We provide strong evidence that visual tokens are in fact highly interpretable, once we adopt the right comparison to contextual LLM embeddings.
%     \item We conduct a controlled study by training a total of 9 MLP projections covering all combinations of three vision encoders and three LLMs, as well studying an off-the-shelf VLM and several ablation training runs.
%     \item We reveal the \textit{Mid-Layer Leap} phenomenon: visual tokens at the LLM input align to mid-layer text embeddings rather than to the corresponding layer.
%     \item We provide a deep dive into what \lens interpretations qualitatively look like. 
% \end{enumerate}

Overall, our findings challenge existing assumptions about the interpretability of visual tokens, and offer new insights about the alignment of vision and language representations.
%Since existing interpretability tools were not up to the task of answering our research questions, we develop \lens as a new tool with diverse and exciting future work.
We encourage the reader to explore the interactive demo and will release \lens as a package with easy access to our database of contextual embeddings to facilitate its adoption.
% \footnote{URL removed for peer review. Demo submitted as zip file.}

% We will release reproducible code, an interactive demo and easy download for our contextual embedding database.


%%% BEFORE Benno rewrite

% Transforming a Large Language Model (LLM) into a Vision-Language Model (VLM) can be as simple as training a linear projection or shallow MLP that maps visual representations into the embedding space of a frozen language model~\citep[\textit{inter alia}]{tsimpoukelli2021multimodal,alayrac2022flamingo,merullo2023linearly,manas2023mapl,liu2023visual,beyer2024paligemma}.
% The empirical success of this approach has been repeatedly established, and the downstream performance of VLMs can be further improved by multiple stages of fine-tuning that update different subsets of the model parameters~\citep[\textcolor{red}{citations++}]{bai2023qwen,cho2025perceptionlm}\fixme{Add additional citations.}.

% Despite the success of training only a simple projection, there is a lack of clarity about how the visual representations are integrated inside the LLM.
% Recent work has investigated this question from the perspective of linear probes~\citep{belinkov2022probing} and sparse autoencoders~\citep[SAE]{cunningham2023sparse}.\fixme{Logit Lens approaches should be mentioned here.}
% The VLM-Lens toolkit allows researchers to train linear probes on internal representations to identify causal mechanisms behind model predictions~\citep{sheta2025behavioral}.
% Sparse autoencoders have been used to study how visual representations are integrated into Gemma-2~\citep{team2024gemma}, showing that the sparse representations only converge to low-error reconstructions deep inside the LLM~\citep{venhoff2025visual}.
% Both of these techniques require further training of either an inexpensive linear probe, or per-layer sparse autoencoders.
% \benno{I wonder if we should also mention here that beyond being zero-shot vs further training, LatentLens also gives you diff kinds of insights}

% In this paper, we propose an alternative that does not rely on any additional training \bk{or prompt engineering}.
% Instead, we use nearest-neighbour cross-modal retrieval to understand the integrations of visual inputs in LLMs.
% We dub this approach \lens, which retrieves embedded representations from a corpus of sentence fragments, and compare it against two baselines: the input embedding matrix and the output embedding matrix (LogitLens).
% \benno{especially with the latest update of events (contextual is the better lens even at the input layer) we should just stick to contextual altogether}
% We verify the success of this technique through human judgment and automated VLM judgment across several combinations of vision encoders and LLMs.
% In contrast to previous work, \lens shows highly interpretable representations in the early layers of the LLM, including even the input layer.
% \benno{We definitely need to emphasize this much more imo! With latest findings, we are now interpretable across *all* layers}
% Our key insight is that neither the embedding matrix nor unembedding matrix (Logit lens) of the LLM are ideal for finding interpretable nearest neighbours, and in fact severely underestimate the interpretability of visual token representations.
% Furthermore, we conduct a suite of ablation studies investigating how the data used to train the linear projection and the depth of the linear projection influence interpretability.
% Finally, we perform causal interventions via patching to study how masking the most/least interpretable tokens affects performance on downstream tasks.

% In summary, we make the following contributions:\fixme{Rewrite this at the end.}
% \begin{enumerate}
%     \item We introduce \lens, a new interpretability tool that explains the integration of visual inputs in LLMs;
%     \item TODO
%     % \item A new explanation of how LLMs integrate visual inputs into the LLM;
%     % \item We are the first to show clear evidence of highly interpretable visual soft prompts;
% \end{enumerate}

% The remainder of this paper is structured as follows: \Cref{sec:background} introduces \mm{Complete...}

% We will release reproducible code, an interactive demo and easy download for our contextual embedding database.


%%% BEFORE Desmond rewrite

%Connecting pre-trained vision encoders to LLMs is a simple and successful recipe to convert text-only LLMs into multi-modal models.
%This is achieved by mapping the visual tokens produced by the visual encoder into the LLM's embedding space and concatenating it with the text prompt (e.g. ``Caption this image'').
% Often both pretrained models (LLM and vision encoder) are kept frozen, or only finetuned in later adaptation stages.
%Surprisingly, despite the LLM being frozen\footnote{\mm{Maybe move the previous sentence here?}} and never having been exposed to any non-linguistic tokens, the LLM can still handle these inputs and solve various vision-and-language tasks \addcites.

%The question of how LLMs can accomplish this has been investigated from various perspectives in the literature: deploy its weights only tuned for language now on vision input?
%What happens at this boundary between vision and language, between two distinct semantic spaces?
%Past work hypothesizes or shows some evidence that the situation is hard to interpret:
%(Visual) soft prompts are not interpretable at the input layer.
%Different modality embeddings live in different narrow cones, i.e. exhibit a modality gap.\siva{discussing all of this here could confuse the reader. Just focus on the interpretability of the visual tokens and logit lens.}
%Logitlens on top of visual tokens provides some coarse-grained insights, but only in later LLM layers.
%SAEs can be used to, but require extensive training and do not tell us X.

%But here is little work on how exactly this happens and few fine-grained tools to interpret visual tokens of an LLM.

%We propose LatentLens...

%Equipped with LatentLens, we critically re-examine past insights and show that:
%Visual soft prompts are often highly interpretable and localized.
%We can find more detailed interp in subsequent layers.
%The so-called modality gap is not a clearly defined issue, we offer counter-evidence of clear token-level alignment (opposed to modality-level).

%Compared to past VL interp work, we go far beyond analysing a couple off-the-shelf models and train various model combinations from scratch.
%Instead of manual eye-balling, we release automatic metrics.
%We release interpretation maps across 12 model combinations across layers, and across different lenses (Input Embedding Matrix, LogitLens, LatentLens).
%For our LatentLens we release a large corpus of contextual text embeddings that can be used to interpret the internal workings of multimodal LLMs.

%We then ask:
%What exactly leads to the high interpretability we observe?
%And how do interpretable tokens affect the behaviour/output of the LLM?
%We conduct a series of experiments.
%We see different trends across different types of vision encoders, and also across LLms. We offer some explanations.
%We change caption length and find...
%We change the task and find...
%Finally, we ask if interpretable tokens are more important for the LLM than non-interpretable ones.
%From patching/removal experiments we find...

%In summary we contribute:
%\begin{enumerate}
%    \item Answers to how LLMs can so easily integrate visual inputs
%    \item First to show clear and across-models evidence of highly interpretable visual soft prompts
%    \item LatentLens, a new interpretability framework/tool/lens for visual tokens inside LLMs. Combined with automatic metrics (human validated), and large corpora of contextual embeddings.
%    \item Extensive ablations and analysis where interp originates from and what role it plays for final behavior of LLMs
%\end{enumerate}


%(Things that could be mentioned:)
%- we are interested in the boundary between perception/continuous inputs and symbols/discrete processing
%- evidence of shared repr between V and L (similar to multi-lingual grand goals)

% Paper flow:

% \begin{enumerate}
%     \item Set the scene - 1) Background on model arch/training, and 2) on existing tools/frameworks for looking into visual tokens (in LLMs)
%     \item  Formally introduce LatentLens as interp method/tool
%     \item Main results: how does LatentLens provide a more-finegrained/better lens into how visual tokens and alignment to llm?
%     \item  Ablations, More detailed analysis: evolution across layers, what do they encode, diff results when we change mapping
%     \item  Going beyond analysis, some ideas how this interp. in practice actually affects model processing? more causal/patching stuff
%     \item  related work (would maybe mention linear probes)
%     \item 
% \end{enumerate}
% Section titles should/could be takeaways (or otherwise subsection titles)

==> sections/2_background_realign.tex <==
\section{Background}
\label{sec:background}
% -----------------------------------------

% We first introduce background on VLMs and prior work on analyzing their latent representations.

% -----------------------------------------
\subsection{Turning LLMs into VLMs}
% -----------------------------------------

A common approach for converting an LLM into a VLM is to project representations produced by a vision encoder into the embedding space of the LLM via a learned connector.
More formally, let \venc be a pre-trained vision encoder, which produces a sequence of \textit{image embeddings} $\venc(\ximg) = \left[\patchvec{1}, \patchvec{2}, \ldots, \patchvec{T_v}\right]$ with $\patchvec{i} \in \mathbb{R}^{d_v}$ for a given image $\ximg$, let \llm be a pre-trained language model, and let $\xtext$ be a textual input.
A multimodal input is constructed as follows: 
First, $\xtext$ is processed by a tokenizer $\tok$ and then converted into token embeddings via an embedding matrix $\mathbf{E}_{\texttt{emb}} \in \mathbb{R}^{\lvert \mathcal{V} \rvert \times d}$.
Second, \textit{visual tokens} representing $\ximg$ are obtained by projecting each image embedding $\patchvec{i}$ into the embedding space of \llm using a projection function\footnote{In practice, $\proj$ is usually a linear layer, an MLP, or an attention-based module ~\cite{liu2023visual, wang2024qwen2vl}.} $\proj: \mathbb{R}^{d_v} \mapsto \mathbb{R}^d$.
Finally, the visual and textual representations are concatenated $\embedding{\mathbf{x}} = [\projvec{1}, \ldots, \projvec{T_v}, \textvec{1}, \ldots, \textvec{T_t}]$, where $\projvec{i} = \proj\left(\patchvec{i}\right) \in \mathbb{R}^{d}~\forall~i = 1, \ldots, T_v$ and $\textvec{1}, \ldots, \textvec{T_t} = \emb(\tok(\xtext)) \in \mathbb{R}^{T_t \times d}$.
The resulting multimodal sequence $\embedding{\mathbf{x}}$ is then processed by the \llm and converted into latent representations $\hlayer{i}{\ell} \in \mathbb{R}^d$, where $i$ denotes the position in the sequence and $\ell$ a layer, respectively.\footnote{Color-coding is used for visual token representations ($\vhidden{i}{\ell}$).}
During the forward pass, textual representations can self-attend to the information encoded in the visual representations $\vhidden{i}{\ell}$.
% \footnote{More specifically, visual information is incorporated into the textual representations via the linear combination of value representations implemented by the self-attention layer. \Fixme{do we need this?}}

% -----------------------------------------
%\paragraph{Training.}
\textbf{Training.}
% -----------------------------------------
%
Given a dataset $\mathcal{D}=\{(\ximg,\xtext)_i\}_{i=1}^N$ of image-caption pairs, the \llm can be trained by minimizing the cross-entropy loss over the target caption tokens:
\vspace{-0.5em}
\[
\mathcal{L}_{\text{LM}} = -\sum_{t=T_{\text{instr}}+1}^{T} \log p(y_t \mid y_{<t}, \ximg),
\] where:
$\tok(\xtext) = [\underbrace{y_1, \ldots, y_{T_{\text{instr}}}}_{\text{instruction}}, \underbrace{y_{T_{\text{instr}}+1}, \ldots, y_{T}}_{\text{caption}}]$, and, unless stated otherwise, only the weights of \proj{} are trained, with the \llm{} and \venc{} weights frozen.

% -----------------------------------------
\subsection{Interpreting VLM representations}
\label{sec:logit-lens}
% -----------------------------------------

An important open question is what exactly is encoded in visual token representations as they are processed by an LLM, and to what extent are the latent visual token representations ($\vhidden{i}{\ell}$) interpretable as language-like tokens?
We will briefly introduce popular approaches for studying these questions.
We note that other supervised or prompting-based approaches exist such as probing \citep{belinkov2022probing}, SAEs \citep{cunningham2023sparse}, LatentQA \citep{pan2024latentqa} or Patchscopes \citep{ghandeharioun-etal-2024-patchscopes}.
% However these methods require training. 
Instead, we focus on methods which are training-free and directly leverage the LLMs representation space. 
% \sonia{I think it's also worth emphasizing that you can use ad hoc embedding spaces (like LLMs and DINO). It's super cool this result transfers and should be more emphasized as a contribution. It's more significant than the "contextual embedding" thing which Gandelsman has already done in his paper to my understanding.}

% -----------------------------------------
%\paragraph{\elens.}
\textbf{\elens.}
% -----------------------------------------
%
The simplest approach to interpret visual token representations is to compare them to the elements of the embedding matrix $\mathbf{E}_{\texttt{emb}}$ of \llm.
This is motivated by the projection layer being trained to output representations that are compatible with the embedding space of \llm. 
For this approach, each $\projvec{i}$ (or its corresponding latent $\vhidden{i}{\ell}$ at layer $\ell$) is compared to the embeddings in \llm's embedding matrix $\mathbf{E}_{\texttt{emb}}$ via cosine similarity and the top-k most similar embeddings serve as ``labels.'' \elens has been previously used for interpreting soft prompts \citep{lester-etal-2021-power}, visual tokens \citep{mokady2021clipcap, jiang2025analyzing} or speech \citep{ogunremi2025transcribe}.

% -----------------------------------------
%\paragraph{\logitlens.}
\textbf{\logitlens.}
% -----------------------------------------
%
A slightly different but conceptually very similar approach is the \logitlens~\citep{logitlens}.
Instead of comparing latent representations directly to embeddings, \logitlens projects the latent representation to the unembedding space of the model by multiplying  $\vhidden{i}{\ell}$ with the unembedding matrix $\mathbf{W}_{\texttt{unemb}} \in \mathbb{R}^{d \times \lvert \mathcal{V} \rvert}$, obtaining a distribution over vocabulary items. 
Then, the top-k vocabulary items, i.e., those with the largest logits, are retrieved as ``labels''.
\logitlens been widely used in previous work analyzing LLMs~\citep{geva-etal-2022-transformer,geva-etal-2023-dissecting,fierro-etal-2025-multilingual}, and has recently been adopted for VLMs \citep{shukor2024implicit, neo2025towards, jiang2025interpreting}.
% \mm{Mention limitations}



==> sections/6_causal.tex <==
% -----------------------------------------
\section{Masking interpretable tokens affect downstream performance}
\label{sec:patching}
% -----------------------------------------

% \bk{Vibe of this section: We believe this is a strong foundational contribution in itself for XYZ reasons.
% But we also want to provide reader with some ideas of how this relates to downstream behavior or further causal insights what drives VLM performance.
% }

Do insights from \lens lead to interesting patching or downstream experiments. \mm{Update intro sentence once the section is finalized.}



While the previous sections established the prevalence of interpretable tokens, it remains unclear whether these features are mechanistically critical for generation or functionally equivalent to non-interpretable ones. 

% -----------------------------------------
\paragraph{Experimental setup.}
% -----------------------------------------

To determine if \textit{interpretable} tokens are functionally distinct, we evaluate their impact on model performance using image captioning as a proxy task. 
We analyze the Olmo-7B model with CLIP VIT-L\%14 as the vision encoder, utilizing contextual similarity at the 8th layer as a proxy for interpretability. 

As demonstrated in \Cref{subsec:eval_interpretability} and \Cref{fig:} (\Fixme{Add this figure}), contextual similarity serves as a robust proxy for interpretability in this architecture. 
We design a masking intervention where specific target tokens are replaced with a "generic" embedding, computed as the global mean of all tokens across the validation set. To quantify impact, we compare two strategies under fixed masking budgets: masking tokens in descending order of contextual similarity (targeting the most interpretable features) versus masking in ascending order (targeting the least interpretable).

% -----------------------------------------
\paragraph{Results.}
% -----------------------------------------

% -----------------------------------------
\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\columnwidth]{figures/patching/masking_budget_vs_interp_values.png}
    \caption{\mm{Update caption.}}
    \label{fig:patching}
\end{figure}
% -----------------------------------------

\Cref{fig:patching} illustrates the resulting degradation in caption quality relative to our baseline score of 6.5. Masking interpretable tokens induces a severe performance drop; at a budget of 0.2, the score falls to 4.65, deteriorating further to 3.6 at a budget of 0.3. In stark contrast, masking non-interpretable tokens results in negligible loss, maintaining a score of 6.2 even at a 0.3 budget. This disparity highlights that tokens identified as "interpretable" are functionally distinct and disproportionately critical for the model's generative capabilities, whereas non-interpretable tokens are largely redundant.
\benno{Let's cite register tokens eg "it is an open questions if these non-interp tokens originally come as register tokens [CITE] out of the vision encoder" and we can optionally also empirically check this}

\benno{Optional but would be very cool: Show some qual. open-vocab segm results: do some clustering of how often words/phrases appear or something}

% 1. we find that tokens can be well separated into interp and non-interp via simple heuristic (see \Cref{tab:ablations})
% --> show figure with cluster (x axis would be input emb., y axis LatentLens), then put datapoints in that humans judged interp or non interp

% 2. we need this heuristic because human label expensive --> patching needs lots of tokens 

% 3. now we can answer RQ: do interp tokens play diff role, are non-interp tokens even needed/used for anything?

% 4. concrete experiments
% a) replace 10,20, 40\% of either interp or non-interp tokens with avg of all tokens (or avg of either interp/non-interp tokens)
% b) do the same but in later layers
% c) patching from one image into another image (if non-interp tokens are task vectors, this should not affect perf much)


% OPTIONAL: 

% \subsection{Making the visual tokens more into language}
% another way to frame this: how close to language are these tokens really? can the LLM copy them? etc

% Similarly to neologism paper, can we introduce a discrete bottleneck:
% We translate the visual tokens into its top-k nearest neighbors, essentially showing the LLM now something like discrete text.
% And if that does degrade performance, can we learn a constant vision task vector that we can add to these text tokens?
% This would essentially show that vision and text are quite easy to disentangle in embedding space

==> sections/behind_anon.tex <==
\section{Behind The Scenes}
\label{app:behind_scenes}
% -----------------------------------------
The goal of this section is to make science more transparent and engaging, showing not just the polished paper at the end but also all the detours and lessons learned.
Note: Due to anonymity certain details are omitted, and will be released at full length for the camera-ready version.

\subsection{From start to finish}
\paragraph{The pivot.} This project started last winter (December 2024) when the first author, originally working on vision-and-language models in general, was determined to pivot towards \textit{understanding} models and fundamental science.
So interpretability was the natural direction to look into, from afar it had been intriguing to follow the field the past few years.
But just doing interpretability for the sake of interpretability did not feel like the right approach.
So what was an actual fundamental question that many people would care about, ourselves included, where interpretability could naturally help?

\paragraph{Brainstorming.} The first author tried to present too many potential ideas at once in their lab meeting.
There was not enough time to present them all, and it would not have been a fun presentation to follow with too many disjoint pitches.
So a lab colleague simply asked:
``Which one of these questions are you genuinely excited about?''
And this is how we ended up with this paper and the research question we ask:
How can frozen LLMs possibly make sense of visual tokens?
Do they look like language tokens to the model?
We started with this simple question but the first author could not have possibly imagined all these new insights we would stumble upon, such is the process of science.
It was really a situation of unknown unknowns:
the kind of experiments and ideas we would eventually end up with were inconceivable at the time, and how with each new experiment, three new options opened up.
As a result writing the paper in 8 pages was very challenging and three sections had to be cut even from the appendix.

\paragraph{Don't trust assumptions.}
If the first author had to take away just one lesson from the project, it would be to never trust long-held assumptions (either by oneself or the field).
We had assumed that visual tokens were not really interpretable with nearest neighbors from the embedding matrix, and several papers hinted in that direction.
In retrospect, we should have simply tested this empirically across several models from day one.
Instead, the first author read papers about anisotropy and other interpretability literature, prematurely concluding that embeddings from different modalities live in entirely different narrow cones.\footnote{We even ran lots of experiments on anisotropy and concluded that effects reported in other papers seemed overly simplified. At this point I wouldn't feel confident saying that different modalities live in different narrow cones inside e.g. an LLM.}
So, then the question became:
If these tokens are not interpretable and live in different subspaces, maybe we have to perform more linear algebra and embedding space tricks to show how they relate to text? Rotate them around, learn some simple mappings, specific subspaces, ...?

\paragraph{The Mosaic Dataset.}
Eventually, the first author hypothesized:
Maybe visual tokens are not directly mapped to interpretable words (measured by NNs from the embedding matrix) because real data is messy?
Visual objects in a scene span many tokens, or a single token might represent several objects and different attributes.
So it would be no surprise that they don't just cleanly map to a single concept.
But what if we could simplify this situation?
What if we could make the data we train on simpler and simpler until we see very predictable nearest neighbors.
This is where the project went ``off-track'' for a while and we started experimenting with toy datasets we coined \textit{Mosaic}, where the model gets as input an image like this:

\begin{figure}[H]
    \centering
    \includegraphics[width=0.25\linewidth]{mosaic.png}
\end{figure}

The LLM would then be trained to predict the sequence of color words one after the other (``red blue red pink ...''), essentially ``copying'' each visual token's corresponding color to the text space.
We observed some interesting quirks, but surprisingly not many interpretable nearest neighbors (i.e. color words from the embedding matrix).
In fact, fewer than on the natural images we report in this paper.
We even ran various causal patching experiments, studied high-norm outliers, etc!
They all seemed interesting at the time, but again, simply testing our assumptions early would have saved us these detours.
At this point we had already adopted the Molmo codebase for training models, since we cared about how \textit{frozen} LLMs make sense of visual tokens.
But most VLMs you can take off-the-shelf unfreeze the LLM weights at some stage of training, which is why we opted for our controlled training setup that the final paper still builds upon.

\paragraph{Hope.}
The first author does not remember when exactly we finally questioned our assumptions, and empirically tested the interpretability on natural images.
But sometime around July, we started exploring interactive demos of natural images with the top NN from the embedding matrix.
Since we happened to explore OLMo+CLIP-ViT, we were surprised to see so many meaningful words.
The cosine similarity was low (between e.g. $0.07$ and $0.15$), much lower than what \lens eventually yields.
Nonetheless this was encouraging, but it soon became clear that automating the judgment of whether an NN is interpretable is not trivial.\footnote{It would take another 3 months to develop the full LLM judge we eventually relied upon.}

\paragraph{A first glimpse of the final story.}
With these exciting findings (40\% to 60\% of tokens in OLMo+CLIP-ViT are interpretable), the initial story of the paper was roughly:
Visual tokens at layer 0 are more interpretable than some would assume!
In the background we kept working on directions that did not end up in the main paper or even appendix:
1) We conducted ablations under which conditions this interpretability would increase or decrease, now in \Cref{app:ablations}, though without any trace of these initial \elens results.
2) We always wondered what these strange non-interpretable tokens encode... They often had the same \elens nearest neighbors, they were often in non-salient background regions. Were they something akin to task vectors or register tokens?
At the time this seemed like an interesting enough story to publish:
Past work assumes visual tokens are rarely interpretable at the input via \elens but here we show for some models that is not the case. We show ablations, we show patching experiments. Some qualitative results.
It is good we kept exploring further:
Some co-authors kept wondering: What happens to visual tokens at LLM layers after the input?
And that's where the final paper we now have started taking shape.
We adopted \elens and \logitlens not just at the beginning or end of the model but throughout.
And eventually we wondered: What if we use contextual embeddings instead of static embedding matrices?

\subsection{Lessons and Reflections}

\paragraph{Automation.}
This project co-occurred with the rise of Cursor and Claude Code.
Especially interactive demos for quick exploration are now much easier to build, crucial for projects like this one.
Due to the speed of experimentation, a lot of ideas on the side did not make it into the paper but can now be easily continued as follow-up work.

\paragraph{Lessons on science.}
As mentioned above, testing the simplest assumptions early on is something the first author will keep as a guiding principle for future research.
The field knows less than one would expect.
Models change constantly, experiments might look different with slightly different setups.
Re-run what others have seemingly done before.

\paragraph{Interpretability is fun.}
The process of open-ended discovery is very enjoyable and naturally leads to interesting brainstorming sessions with colleagues and friends.
The first author highly recommends working at least on one interpretability project in one's research journey.
The community is quite unique, reflective and open to good ideas (ideally) regardless of whether they are immediately useful downstream.


==> sections/logit_lens_limitations.tex <==
% -----------------------------------------
\section{Pitfalls of logit lens}
\label{sec:logit-lens-limitations}
% -----------------------------------------

\begin{itemize}
    \item 
\end{itemize}

==> sections/notation.tex <==
% ============================================================================
% Multimodal LLM Notation Macros
% ============================================================================
% Usage: Include this file in your main document with \input{macros}
% Required packages: xcolor, amsmath, amssymb, xspace
% ============================================================================

% Add xspace to required packages
\RequirePackage{xspace}

% ----------------------------------------------------------------------------
% Color Definitions
% ----------------------------------------------------------------------------
\definecolor{visioncolor}{RGB}{46, 125, 50}      % Green for vision
\definecolor{languagecolor}{RGB}{13, 71, 161}    % Blue for language
\definecolor{connectorcolor}{RGB}{191, 54, 12}   % Orange for connector
\definecolor{inputcolor}{RGB}{123, 31, 162}      % Purple for inputs
\definecolor{embeddingcolor}{RGB}{194, 24, 91}   % Pink for embeddings
\definecolor{blackcolor}{RGB}{0, 0, 0}           % Black for tokenizer/embedder

% ----------------------------------------------------------------------------
% Semantic Color Commands
% ----------------------------------------------------------------------------
% Use these to wrap text/math in semantic colors
\newcommand{\vision}[1]{\textcolor{visioncolor}{#1}}
\newcommand{\llmtext}[1]{\textcolor{languagecolor}{#1}}
\newcommand{\connector}[1]{\textcolor{connectorcolor}{#1}}
\newcommand{\inputdata}[1]{\textcolor{inputcolor}{#1}}
\newcommand{\embedding}[1]{\textcolor{embeddingcolor}{#1}}
\newcommand{\blacktext}[1]{\textcolor{blackcolor}{#1}}

% ----------------------------------------------------------------------------
% Model Components (use in text or math mode)
% ----------------------------------------------------------------------------
% Vision encoder
\newcommand{\venc}{\vision{\texttt{venc}}\xspace}

% Language model
\newcommand{\llm}{\llmtext{\texttt{llm}}\xspace}

% Connector/projector
\newcommand{\proj}{\connector{\texttt{proj}}\xspace}

% Embedding layer
\newcommand{\emb}{\blacktext{\texttt{emb}}\xspace}

% Tokenizer
\newcommand{\tok}{\blacktext{\texttt{tok}}\xspace}

% ----------------------------------------------------------------------------
% Input Data (use in math mode with $...$)
% ----------------------------------------------------------------------------
% Input image
\newcommand{\ximg}{\inputdata{x_{\text{img}}}\xspace}

% Input text
\newcommand{\xtext}{\inputdata{x_{\text{text}}}\xspace}

% Target text
\newcommand{\ytext}{\inputdata{y_{\text{text}}}\xspace}

% ----------------------------------------------------------------------------
% Embedding Space Representations (use in math mode with $...$)
% ----------------------------------------------------------------------------
% Visual prefix tokens (VPT) sequence
\newcommand{\vpt}{\embedding{v}}

% Text embeddings sequence
\newcommand{\tpt}{\embedding{t}}

% Combined input sequence
\newcommand{\zseq}{\embedding{z}}

% Embedding dimension
\newcommand{\dimemb}{\embedding{d}}

% ----------------------------------------------------------------------------
% Parameters (use in math mode with $...$)
% ----------------------------------------------------------------------------
% Vision encoder parameters
\newcommand{\thetav}{\vision{\theta_v}}

% Language model parameters
\newcommand{\thetal}{\llmtext{\theta_\ell}}

% Projector parameters
\newcommand{\thetap}{\connector{\theta_p}}

% ----------------------------------------------------------------------------
% Individual Token Vectors (use in math mode with $...$)
% ----------------------------------------------------------------------------
% Patch representation vector (e.g., \patchvec{i} or \patchvec{1})
\newcommand{\patchvec}[1]{\vision{\mathbf{v}_{#1}}}

% Projected visual token vector (e.g., \projvec{i} or \projvec{1})
\newcommand{\projvec}[1]{\connector{\mathbf{p}_{#1}}}

% Text token embedding vector (e.g., \textvec{j} or \textvec{1})
\newcommand{\textvec}[1]{\llmtext{\mathbf{e}_{#1}}}

% Hidden representation at position i, layer l (generic, uncolored)
\newcommand{\hlayer}[2]{\mathbf{h}_{#1}^{(#2)}}

% Visual token hidden representation at position i, layer l (colored orange/red, same as projector output)
\newcommand{\vhidden}[2]{\connector{\mathbf{h}_{#1}^{(#2)}}}

% Generic reference vector (uncolored)
\newcommand{\refvec}[1]{\mathbf{r}_{#1}}

% Contextualized text reference vector at position j, layer l (colored blue)
\newcommand{\tref}[2]{\llmtext{\mathbf{r}_{#1}^{(#2)}}}

% ============================================================================
% Usage Examples:
% ============================================================================
% 
% In text: The \venc encodes images...
% 
% Vision encoding:
% $\venc(\ximg) = [\patchvec{1}, \patchvec{2}, \ldots, \patchvec{T_v}]$
%
% Projection:
% $\proj(\patchvec{i}) = \projvec{i}$
%
% Text embedding:
% $\emb(\tok(\xtext)) = [\textvec{1}, \textvec{2}, \ldots, \textvec{T_t}]$
%
% Combined sequence:
% $\zseq = [\projvec{1}, \ldots, \projvec{T_v}, \textvec{1}, \ldots, \textvec{T_t}]$
%
% Forward pass:
% $p(y \mid \ximg, \xtext) = \llm(\zseq)$
%
% Training objective:
% $\thetap^* = \arg\min_{\thetap} \mathcal{L}(\llm([\proj_{\thetap}(\venc(\ximg)); \emb(\tok(\xtext))]), \ytext)$
%
% ============================================================================
